Exploring Sub-skeleton Trajectories for Interpretable Recognition of Sign Language

Recent advances in tracking sensors and pose estimation software enable smart systems to use trajectories of skeleton joint locations for supervised learning. We study the problem of accurately recognizing sign language words, which is key to narrowing the communication gap between hard and non-hard of hearing people. Our method explores a geometric feature space that we call `sub-skeleton' aspects of movement. We assess similarity of feature space trajectories using natural, speed invariant distance measures, which enables clear and insightful nearest neighbor classification. The simplicity and scalability of our basic method allows for immediate application in different data domains with little to no parameter tuning. We demonstrate the effectiveness of our basic method, and a boosted variation, with experiments on data from different application domains and tracking technologies. Surprisingly, our simple methods improve sign recognition over recent, state-of-the-art approaches.

==> figures/seq_eg.tex <==
% \begin{figure}[H]\centering \vspace{-.3cm}  
\begin{figure}[t]\centering %\vspace{-.3cm}  
  \begin{subfigure}[t]{.69\columnwidth}
    \includegraphics[width=\columnwidth,height=.25\columnwidth]{./figures/LM_seq_eg.png}
    \caption{LM right/left hand joints for sign \textit{coat}.}
  \end{subfigure}
%   \includegraphics[width=\columnwidth,height=.25\columnwidth]{./figures/LM_seq_eg.png} 
  \begin{subfigure}[t]{0.3\columnwidth}
    \includegraphics[width=0.8\columnwidth,height=.85\columnwidth]{./figures/KinTrans_seq_eg.png}
    \caption{KinTrans upper body joints for sign \textit{credit card}.}
  \end{subfigure}
  \hfill
%   \begin{subfigure}[b]{0.25\columnwidth}
%     \includegraphics[width=0.7\columnwidth,height=.85\columnwidth]{./figures/NTU_seq_eg.png}
%     \caption{NTU RGB+D full body joints for action \textit{cheer up}.}
%   \end{subfigure}
%\vspace{-.7cm}	
\todo[inline]{Split Fig in subsections}
\caption{
Human skeletal joint examples showing movement from earlier (lighter) to later (darker) time frames. See Section~\ref{sec:exp_res:datasets} for data set details.}
	\label{fig:seq_eg} 
%  	\vspace{-.3cm}
\end{figure}


==> figures/testtime.tex <==
\begin{figure}[p]

\begin{tikzpicture}    %[scale=.65]
\pgfplotsset{every axis title/.append style={at={(0.5,0.85)}}}
\begin{groupplot}[
     group style = {group size = 2 by 2,
                    horizontal sep=1.25cm,
                    vertical sep=0.15cm,},
     width= .52\columnwidth, %5.5cm,
     height= .32\columnwidth, %3.6cm,
     grid style=dashed,
     xmode = normal,
     xmin=0.8, xmax=5.2,
     xtick style={draw=none},
     xtick=data,
     xticklabels={,,},
     ybar,
     ymajorgrids=true,
     ymode = log,
     log ticks with fixed point,
     log origin = infty,
    ]

\nextgroupplot[
sharp plot,
stack plots = false,
% legend pos= south east, %outer north east,
ymin=8, ymax=1300,
ytick={1,10,100,1000,10000},
yticklabels={$1$,$10$,$100$,$10^{3}$},
ylabel={Time [ms]},
% title={Test Sequence Latency},
ylabel shift = -0.20cm,
y tick label style={font=\small},
% legend pos= south east, %outer north east,
legend style={
    at={(2.262,0.98)},
    font=\small
    },
% height=.5\columnwidth,%3.6cm,
% legend columns=2,
]

\addplot[
color=blue,
mark=o,
]
coordinates {(1,51.9)(2,66.2)(3,68.7)(4,61.6)(5,69.6)};

\addplot[
color=blue,
mark=x,
]
coordinates {(1,25.3)(2,32.76)(3,29.6)(4,32.9)(5,34.5)};

\addplot[
color=blue,
mark=square,
]
coordinates {(1,12.6)(2,19.7)(3,23.6)(4,50.1)(5,103.0)};

\addplot[
color=black,
mark=triangle,
]
coordinates {(1,16.5)(2,27.3)(3,30.1)(4,74.8)(5,163.2)};

\addplot[
color=black,
mark=+,
]
coordinates {(1,41.1)(2,92.4)(3,130.8)(4,115.1)(5,582.9)};

\legend{1NN-s CF}
\addlegendentry{1NN-s CF-apx}
\addlegendentry{1NN-s DTW}
\addlegendentry{DM-s DTW}
\addlegendentry{DM-m DTW}


\nextgroupplot[group/empty plot
]

\nextgroupplot[
sharp plot,
stack plots = false,
xticklabels={$2$, $3$, $5\%$, $10\%$, $20\%$},
xlabel={Trainers per class},
ymode = normal,
ymin=68, ymax=102,
ytick={60,70,75,80,85,90,95,100},
yticklabels={$60$,$70$,$75$,$80$,$85$,$90$,$95$,$100$},
ylabel={Accuracy~[\%]},
ylabel shift = -0.20cm,
x tick label style={font=\small},
y tick label style={font=\small},
xticklabel shift = -0.10cm,
xlabel shift = -0.10cm,
]

\addplot[
color=blue,
mark=o,
]
coordinates {(1,70.5)(2,79.0)(3,79.1)(4,94.4)(5,97.4)};

\addplot[
color=blue,
mark=x,
]
coordinates {(1,69.9)(2,74.2)(3,75.2)(4,93.1)(5,96.5)};

\addplot[
color=blue,
mark=square,
]
coordinates {(1,79.1)(2,83.9)(3,90.1)(4,98.0)(5,99.3)};

\addplot[
color=black,
mark=triangle,
]
coordinates {(1,77.9)(2,87.4)(3,92.7)(4,97.9)(5,99.5)};

\addplot[
color=black,
mark=+,
]
coordinates {(1,80.6)(2,89.6)(3,92.2)(4,98.4)(5,99.8)};


\nextgroupplot[
sharp plot,
stack plots = false,
xticklabels={$2$, $3$, $5\%$, $10\%$, $20\%$},
xlabel={Trainers per class},
ymin=0.05, ymax=15000,
ytick={0.1,1,10,100,1000,10000,100000},
yticklabels={$0$,$1$,$10$,$100$,$10^{3}$,$10^{4}$},
ylabel={Distances [1]},
ylabel shift = -0.20cm,
x tick label style={font=\small},
y tick label style={font=\small},
xticklabel shift = -0.10cm,
xlabel shift = -0.10cm,
% height=3.6cm,
]

\addplot[
color=blue,
mark=o,
]
coordinates {(1,0.7)(2,1.0)(3,1.2)(4,0.8)(5,0.9)};

\addplot[
color=blue,
mark=x,
]
coordinates {(1,0.1)(2,0.1)(3,0.1)(4,0.1)(5,0.1)};

\addplot[
color=blue,
mark=square,
]
coordinates {(1,146)(2,219)(3,236)(4,511)(5,1028)};

\addplot[
color=black,
mark=triangle,
]
coordinates {(1,146)(2,219)(3,236)(4,511)(5,1028)};

\addplot[
color=black,
mark=+,
]
coordinates {(1,438)(2,876)(3,1180)(4,1022)(5,5140)};

\end{groupplot}

\end{tikzpicture}
\caption{Query latency of our classifiers for various training sets sizes using the KinTrans data set.
Shown are average time per query (top), overall classification accuracy (bottom left), and average number of trajectory distance computations per query (bottom right).
}


\label{fig:testtime}
\end{figure}




==> tables/accuracy_human_action.tex <==
% \begin{table}[p]

% \end{table}



==> tables/accuracy_lm.tex <==
\begin{table}[]
  \centering
{
\begin{tabular}{l|llr}
\thickhline
Benchmark                         & Paper                 & Method               & Accuracy        \\ \thickhline
\multirow{5}{*}{LM - 5-fold XSub} & \citet{hernandez2020}\footnote{Sequences are generated from a non-publicly available manual segmentation process.} & Kine.-LSTM           & $91.1$          \\ \cline{2-4} 
                                  & \multirow{4}{*}{Ours\footnote{Sequences are generated from our automatic segmentation process.}} & NN-s                 & $83.2$          \\
                                  &                       & $k$NN-s ($k=20$)     & $83.4$          \\
                                  &                       & DM-m                 & $93.1$          \\
                                  &                       & DM-m (multi-joint $C$) & \textbf{93.8} \\ \thickhline
\end{tabular}
}
\caption{LM American sign language data set classification accuracy results comparing our methods against \citet{hernandez2020}.
}
	\label{tab:accuracy_lm}
\end{table}


% \begin{tabular}{l|llr}
% \thickhline
% Benchmark                      & Method & Paper & Accuracy      \\ \thickhline
% \multirow{3}{*}{LM - 5-fold XSub}            & Kine.-LSTM & \citet{hernandez2020}      & $91.1$          \\ \cline{2-4} 
%                               & NN-s & Ours      & $83.2$          \\
%                               & $k$NN-s ($k=20$) & Ours      & $83.4$          \\
%                               & DM-m & \textbf{Ours}      & \textbf{93.8} \\ \thickhline
% \end{tabular}

==> tables/crit_subskel.tex <==
\begin{table}[h]
  \centering
{
\begin{tabular}{llll|lcrrc}
\hline
\multicolumn{4}{c|}{Mining Input}      & \multicolumn{5}{c}{Feature Template Result} \\ \hline
Benchm.   & $\mathbb{D}_r$  & Method & $|C|$  & Dist.  & T~~R~~L~~P                 & AJ    & RJ       & DM Class.     \\ \hline
KinTrans  & $20\%$          & NN-s   & $100$  & DTW    & N~N~N~N                    & $5$   & $0$      & -             \\
LM        & $15$/class      & NN-s   & $73$   & CF     & \textbf{Y}~N~N~N           & $2$   & $5$      & -             \\
NTU60     & cam. $2\&3$     & DM-m   & $90$   & DTW    & \textbf{Y}~\textbf{Y}~N~N  & $5$   & $4$      & SVM           \\
UCF       & $15$/class      & DM-m   & $225$  & DTW    & N~N~N~N                    & $3$   & $2$      & Sub. Disc.    \\
MHAD      & $7$ subjects    & NN-s   & $225$  & CF     & \textbf{Y} N N \textbf{Y}  & $0$   & $5$      & -             \\ \hline
\end{tabular}
}
\todo[inline]{End with a nice looking table :D}
\caption{A subset of feature template mining results for various benchmarks. 
Mining input columns show: data set benchmark, training set protocol, our classifier method, and the number of canonical sub-skeletons.
Feature template result columns show selected: distance similarity measure, normalizations (Translate, Rotate, Limb length, at-rest Pose), total numbers of Absolute and Relative Joints, and Distance Matrix classifier.}
	\label{tab:crit_subskel}
	\vspace{-0.35cm}
\end{table}

